Independent dominating sets in planar triangulations

In 1996, Matheson and Tarjan proved that every near planar triangulation on $n$ vertices contains a dominating set of size at most $n/3$, and conjectured that this upper bound can be reduced to $n/4$ for planar triangulations when $n$ is sufficiently large. In this paper, we consider the analogous problem for independent dominating sets: What is the minimum $\epsilon$ for which every near planar triangulation on $n$ vertices contains an independent dominating set of size at most $\epsilon n$? We prove that $2/7 \leq \epsilon \leq 5/12$. Moreover, this upper bound can be improved to $3/8$ for planar triangulations, and to $1/3$ for planar triangulations with minimum degree 5.

==> Figures/gadget-odd-vertices.tex <==
\begin{tikzpicture}[scale=1]
\node (center) [] at (0,0) {};
\node (1) [black vertex] at ($(center) + (90:2)$) {};
\node (2) [black vertex] at ($(center) + (210:2)$) {};
\node (3) [black vertex] at ($(center) + (330:2)$) {};

\node (center) [] at (0,0) {};
\node (a) [red vertex] at ($(center) + (90:.5)$) {};
\node (b) [red vertex] at ($(center) + (210:.5)$) {};
\node (c) [red vertex] at ($(center) + (330:.5)$) {};

\draw[line width=1.3pt] (a) -- (b) -- (c) -- (a);

\node (12) [black vertex] at ($0.5*(1) + 0.5*(2)$) {};
\node (23) [black vertex] at ($0.5*(2) + 0.5*(3)$) {};
\node (13) [black vertex] at ($0.5*(1) + 0.5*(3)$) {};

\draw[line width=1.3pt] (1) -- (12) -- (2) -- (23) -- (3) -- (13) -- (1);

\draw[line width=1.3pt] (1) -- (a) (2) -- (b) (3) -- (c);

\draw[line width=1.3pt] (a) -- (12) -- (b) -- (23) -- (c) -- (13) -- (a);
\end{tikzpicture}

